Deep-field Metacalibration

We introduce deep-field metacalibration, a new technique that reduces the pixel noise in metacalibration estimators of weak lensing shear signals by using a deeper imaging survey for calibration. In standard metacalibration, when estimating the object's shear response, extra noise is added to correct the effect of shearing the noise in the image, increasing the uncertainty on shear estimates by ~ 20%. Our new deep-field metacalibration technique leverages a separate, deeper imaging survey to calculate calibrations with less degradation in image noise. We demonstrate that weak lensing shear measurement with deep-field metacalibration is unbiased up to second-order shear effects. We provide algorithms to apply this technique to imaging surveys and describe how to generalize it to shear estimators that rely explicitly on object detection (e.g., metacalibration). For the Vera C. Rubin Observatory Legacy Survey of Space and Time (LSST), the improvement in weak lensing precision will depend on the somewhat unknown details of the LSST Deep Drilling Field (DDF) observations in terms of area and depth, the relative point-spread function properties of the DDF and main LSST surveys, and the relative contribution of pixel noise vs. intrinsic shape noise to the total shape noise in the survey. We conservatively estimate that the degradation in precision is reduced from 20% for metacalibration to ~ 5% or less for deep-field metacalibration, which we attribute primarily to the increased source density and reduced pixel noise contributions to the overall shape noise. Finally, we show that the technique is robust to sample variance in the LSST DDFs due to their large area, with the equivalent calibration error being ~ 0.1%. The deep-field metacalibration technique provides higher signal-to-noise weak lensing measurements while still meeting the stringent systematic error requirements of future surveys.

==> Makefile <==

texfile := deepfieldmcal
default: pdf-nobib

bib:
	bibtex ${texfile}

pdf-nobib:
	pdflatex ${texfile}
	pdflatex ${texfile}

pdf:
	pdflatex ${texfile}
	bibtex ${texfile}
	pdflatex ${texfile}
	pdflatex ${texfile}

diff:
	latexdiff --graphics-markup=off --disable-citation-markup --math-markup=1 --no-del ${texfile}_v1.tex ${texfile}.tex > ${texfile}_diff.tex
	pdflatex ${texfile}_diff
	bibtex ${texfile}_diff
	pdflatex ${texfile}_diff
	pdflatex ${texfile}_diff

all: pdf diff

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.out \
	${texfile}.ps \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.log \
	${texfile}.fdb_latexmk \
	${texfile}.fls \
	${texfile}.brf

